Typhoon ASR Edge: A 33M-Parameter Thai Speech Recognition Model with Decode-Time Keyword Boosting

While open-weight Thai automatic speech recognition (ASR) has achieved strong general accuracy, the most accurate models require GPUs for real-time or high-concurrency use and fail on domain-specific named entities, such as product names, personal names, and rare words. In addition, Thai is written without spaces between words and permits multiple accepted spellings across Thai and Latin scripts, which prevents standard whitespace-based word spotting from being applied directly. We present Typhoon ASR Edge, a 33M-parameter FastConformer transducer with an auxiliary connectionist temporal classification (CTC) head, along with Typhoon Keyword Boosting, which spots listed keywords on the CTC posteriors, verifies each candidate under both heads, and rewrites only the verified spans of the transcript at decode time. Despite having only 33M parameters, Typhoon ASR Edge provides character error rates (CER) comparable to 115M- to 0.6B-parameter open-weight models on general Thai benchmarks. With a keyword list, Typhoon Keyword Boosting raises entity recall from 32.7% to 87.8%, within three percentage points of the strongest proprietary cloud service. Furthermore, a Rust inference engine runs both acoustic inference and keyword boosting with high throughput and low latency on x86-64 CPUs with Intel AMX, with support for other CPU architectures. The model weights, Typhoon Keyword Boosting, and the Rust inference engine are publicly released.

==> fig_corpus.tex <==
% Figure: plain-transcription CER vs model size for every measured model, same corpus (data = Table tab:cer).
% x = log10(params in M); markers: circle = Whisper, diamond = Qwen3-ASR, square = FastConformer; hollow = stock Qwen.
\usetikzlibrary{shapes.geometric}
\colorlet{famW}{tyWarmDark}
\colorlet{famQ}{tyNeutral}
\colorlet{famF}{tyAccent}
\tikzset{
  pW/.style={circle, fill=famW, inner sep=0pt, minimum size=4.2pt},
  pQ/.style={diamond, fill=famQ, inner sep=0pt, minimum size=5.6pt},
  pQs/.style={diamond, draw=famQ, fill=white, thick, inner sep=0pt, minimum size=5.6pt},
  pF/.style={rectangle, fill=famF, inner sep=0pt, minimum size=4pt},
  plab/.style={font=\tiny, text=black!70, inner sep=1pt},
  pax/.style={font=\scriptsize, text=black!55}}
% #1 = y of the gs2/TVSpeech panel origin, #2..: drawn by the macro below
\newcommand{\corpuspanel}[5]{% #1 title, #2 ymin, #3 ymax, #4 ystep, #5 points
\begin{scope}[x=2.55cm, y=#4, shift={(-1.35,-#2)}]
  \draw[black!35] (1.35,#2) -- (3.5,#2);
  \draw[black!35] (1.35,#2) -- (1.35,#3);
  \foreach \lx/\lab in {1.477/30M, 2/100M, 2.477/300M, 3/1B} {
    \draw[black!35] (\lx,#2) -- ++(0,-0.06cm);
    \node[pax, anchor=north] at (\lx,#2) {\lab};
  }
  \node[font=\footnotesize\bfseries, text=black!70, anchor=south west] at (1.35,#3) {#1};
  #5
\end{scope}}
\begin{figure}[!htb]\centering
\begin{tikzpicture}
% ---------------- left: gigaspeech2-typhoon
\corpuspanel{gigaspeech2-typhoon CER}{4}{9.5}{0.62cm}{
  \foreach \yy in {4,5,6,7,8,9} {\draw[black!35] (1.35,\yy) -- ++(-0.06cm,0); \node[pax, anchor=east] at (1.35,\yy) {\yy};}
  \draw[-{Stealth[length=1.4mm]}, black!35, thin] (3.316,6.09) -- (3.316,4.98);
  \draw[-{Stealth[length=1.4mm]}, black!35, thin] (2.903,8.20) -- (2.903,5.18);
  \node[pQs] at (3.316,6.09) {}; \node[plab, anchor=west] at (3.34,6.09) {Qwen3-ASR-1.7B};
  \node[pQs] at (2.903,8.20) {}; \node[plab, anchor=west] at (2.93,8.20) {Qwen3-ASR-0.6B};
  \node[pW] at (3.190,4.69) {}; \node[pW] at (2.886,4.81) {};
  \node[pQ] at (3.316,4.86) {}; \node[pQ] at (2.903,5.06) {};
  \node[plab, anchor=north] at (3.10,4.62) {Whisper, Qwen-ctx};
  \node[pF] at (2.061,6.89) {}; \node[plab, anchor=north] at (2.061,6.80) {realtime};
  \node[pF] at (1.519,7.20) {}; \node[plab, anchor=west, text=tyAccentDark] at (1.55,7.20) {\textbf{edge}};
  \node[pF, fill=white, draw=famF, thick] at (1.519,8.75) {}; \node[plab, anchor=west] at (1.55,8.75) {streaming};
  \node[pF] at (2.130,8.54) {}; \node[plab, anchor=west] at (2.16,8.54) {nemo-ctc};
}
% ---------------- right: TVSpeech
\begin{scope}[xshift=6.9cm]
\corpuspanel{TVSpeech CER}{6}{14}{0.427cm}{
  \foreach \yy in {6,8,10,12,14} {\draw[black!35] (1.35,\yy) -- ++(-0.06cm,0); \node[pax, anchor=east] at (1.35,\yy) {\yy};}
  \draw[-{Stealth[length=1.4mm]}, black!35, thin] (3.316,10.63) -- (3.316,7.05);
  \draw[-{Stealth[length=1.4mm]}, black!35, thin] (2.903,11.45) -- (2.903,7.48);
  \node[pQs] at (3.316,10.63) {}; \node[pQs] at (2.903,11.45) {};
  \node[pW] at (3.190,6.32) {}; \node[pW] at (2.886,7.66) {};
  \node[pQ] at (3.316,6.87) {}; \node[pQ] at (2.903,7.28) {};
  \node[plab, anchor=west] at (3.34,10.63) {Qwen3-ASR-1.7B};
  \node[plab, anchor=west] at (2.93,11.45) {Qwen3-ASR-0.6B};
  \node[pF] at (2.061,9.92) {}; \node[plab, anchor=north] at (2.061,9.80) {realtime};
  \node[pF] at (1.519,10.59) {}; \node[plab, anchor=west, text=tyAccentDark] at (1.55,10.59) {\textbf{edge}};
  \node[pF, fill=white, draw=famF, thick] at (1.519,13.52) {}; \node[plab, anchor=west] at (1.55,13.52) {streaming};
  \node[pF] at (2.130,13.46) {}; \node[plab, anchor=west] at (2.16,13.46) {nemo-ctc};
  \node[plab, anchor=north] at (3.05,6.12) {Whisper, Qwen-ctx};
}
\end{scope}
% ---------------- legend
\begin{scope}[shift={(-0.2,-0.75)}]
  \node[pW] at (0,0) {}; \node[plab, anchor=west, font=\scriptsize] at (0.1,0) {Whisper fine-tunes};
  \node[pQ] at (3.0,0) {}; \node[plab, anchor=west, font=\scriptsize] at (3.1,0) {Qwen3-ASR fine-tunes};
  \node[pQs] at (6.4,0) {}; \node[plab, anchor=west, font=\scriptsize] at (6.5,0) {stock Qwen3-ASR};
  \node[pF] at (9.2,0) {}; \node[plab, anchor=west, font=\scriptsize] at (9.3,0) {FastConformer};
  \node[pF, fill=white, draw=famF, thick] at (11.5,0) {}; \node[plab, anchor=west, font=\scriptsize] at (11.6,0) {streaming, 0.48\,s};
\end{scope}
\end{tikzpicture}
\caption{\textbf{One corpus, many models.} Plain-transcription CER against
parameter count, log scale, for every measured model of \Cref{tab:cer}. All
filled markers are trained on the same 10{,}846-hour corpus; arrows lead
from stock Qwen3-ASR to its fine-tune. Models with an autoregressive decoder
form one band whatever their family, the transducers a second, and the
greedy CTC model sits above both.}
\label{fig:corpus}
\end{figure}


==> fig_labels.tex <==
% Figure: consensus relabeling of the training corpus (Section 3.2).
% Graphic: figures/ (PDF exported from figures_svg/*.svg). Original TikZ code kept in figures_svg/tikz_original/.
\begin{figure}[!htb]\centering
\includegraphics[width=\linewidth]{figures/fig_labels.pdf}
\caption{\textbf{Consensus relabeling of the training corpus.} We use the Typhoon Whisper Large V3 transcript as the base text (1) and treat any span where the other two teachers differ as a candidate replacement (2). A gradient-boosted arbiter trained on 1{,}041 human-verified utterances scores each candidate and replaces the base span when $p \ge 0.5$ (3). Utterances where the teachers still disagree with the resulting label (mean CER $> 0.16$) are discarded (4).}
\label{fig:labels}
\end{figure}


==> fig_pipeline.tex <==
% Figure: the keyword-boosting system as a top-to-bottom flow, one full-width row per step (Section 5).
% Worked example throughout: the second utterance of Figure 1, เกลือไกล (base text) -> เกริกไกร (listed name).
\begin{figure}[!t]\centering
\newcommand{\wtitle}[1]{{\footnotesize\bfseries\color{black!80}#1}}
\newcommand{\stitle}[1]{{\footnotesize\bfseries\color{tyAccentDark}#1}}
\begin{tikzpicture}[scale=0.9, every node/.append style={transform shape},
  font=\footnotesize,
  row/.style={rounded corners=4pt, draw=black!30, fill=black!4, minimum width=15.9cm, inner sep=0pt, anchor=north west},
  srow/.style={row, draw=tyAccentDark, fill=tyAccentFill},
  what/.style={anchor=north west, inner sep=8pt, text width=3.3cm, align=left, font=\scriptsize, text=black!75},
  box/.style={rounded corners=3pt, align=center, minimum height=7mm, inner sep=3pt, draw=black!40, fill=white, font=\scriptsize},
  note/.style={font=\tiny, text=black!55, inner sep=1pt},
  th/.style={font=\scriptsize\thaifont, inner sep=1pt},
  chip/.style={draw=tyAccent, fill=white, rounded corners=5pt, inner xsep=4pt, inner ysep=1.5pt, font=\scriptsize\thaifont},
  dchip/.style={chip, draw=black!25, text=black!50, font=\scriptsize},
  cell/.style={minimum size=2.4mm, inner sep=0pt, draw=white, line width=0.4pt},
  bar/.style={fill=black!25, minimum height=1.5mm, inner sep=0pt, anchor=west},
  a/.style={-{Stealth[length=1.7mm]}, black!60, semithick},
  da/.style={a, dashed},
  spine/.style={-{Stealth[length=3.2mm, width=3.2mm]}, tyAccentDark, line width=1.8pt}]
% ======================= row 1: encoder
\node[row, minimum height=1.55cm] (r1) at (0,0) {};
\node[what] at (r1.north west) {\wtitle{Encoder}\\one pass per utterance, offline or streaming with a 0.96\,s look-ahead};
\begin{scope}[yshift=-0.15cm, xshift=0.15cm]
\node[box] (aud) at (5.2,-0.62) {audio, 16\,kHz};
\node[box] (enc) at (8.3,-0.62) {FastConformer encoder\\[-1pt]{\tiny 16 layers, $d{=}256$, 33M}};
\node[box] (fr) at (11.9,-0.62) {encoder frames\\[-1pt]{\tiny one per 80\,ms}};
\draw[a] (aud) -- (enc); \draw[a] (enc) -- (fr);
\end{scope}
% ======================= row 2: two heads
\begin{scope}[yshift=-0.85cm]
\node[row, minimum height=3.2cm] (r2) at (0,-1.45) {};
\node[what] at (r2.north west) {\wtitle{Two heads}\\the transducer commits to one transcript; the CTC head keeps every piece at every frame};
\begin{scope}[yshift=-0.15cm, xshift=0.15cm]
\node[box] (tdt) at (5.2,-2.0) {transducer head\\[-1pt]{\tiny beam 8}};
\node[th, anchor=west] (bt) at (6.6,-2.0) {base text:\; นี่พี่ตกใจมากเลยนะเนี่ยที่คุณ\textcolor{tyWarmDark}{เกลือไกล}เขาบอกว่าน้อง\textcolor{tyWarmDark}{กล้อง}เป็นลูกของเขาอ่ะ};
\node[note, anchor=west] at (6.6,-2.35) {the output when no list is given; unseen names come out as similar-sounding words};
\node[box] (ctc) at (5.2,-3.3) {CTC head\\[-1pt]{\tiny posteriors $T{\times}2049$}};
\begin{scope}[shift={(6.75,-3.05)}]
  \foreach \r in {0,...,3} {\foreach \c in {0,...,27} {\node[cell, fill=black!8] at ({\c*0.26},{-\r*0.22}) {};}}
  \foreach \c/\r in {2/1,3/0,5/2,7/3,9/1,10/1,12/0,14/2,15/2,17/3,19/1,21/0,22/2,24/1,26/3} {\node[cell, fill=black!30] at ({\c*0.26},{-\r*0.22}) {};}
  \foreach \c/\r in {12/2,13/2,14/3,15/3} {\node[cell, fill=tyAccent!45] at ({\c*0.26},{-\r*0.22}) {};}
  \node[note, anchor=west] at ({28*0.26},-0.33) {$\leftarrow$ 2,049 pieces};
  \node[note, anchor=north] at ({13.5*0.26},-0.8) {frames $\rightarrow$};
  \node[note, anchor=north, text=tyAccentDark] at ({12.5*0.26},-1.02) {the pieces of \textthai{เกริกไกร} still carry probability mass here, although none was the top piece at its frame};
\end{scope}
\draw[a] (fr.south) -- ++(0,-0.8) -| (tdt.north);
\draw[a] (fr.south) -- ++(0,-0.8) -| ([xshift=-2mm]ctc.north west) -- ([xshift=-2mm]ctc.north west |- ctc.west) -- (ctc.west);
\end{scope}
\end{scope}
% ======================= row 3: search
\begin{scope}[yshift=-1.70cm]
\node[srow, minimum height=3.85cm] (r3) at (0,-4.55) {};
\node[what] at (r3.north west) {\stitle{1\quad Search}\\for each name in the list, slide it along the CTC posteriors and keep the position where its pieces fit best; Latin entries first get Thai forms};
\begin{scope}[yshift=-0.15cm, xshift=0.15cm]
% the posterior strip (same matrix as above), with the name's pieces as a template slid along it
\node[box, anchor=west, align=left, text width=2.45cm] (klist) at (3.95,-5.55) {\textbf{keyword list}\\[1pt]{\thaifont\scriptsize\textcolor{tyAccentDark}{เกริกไกร}\; \textcolor{tyAccentDark}{ก้อง}}\\[-1pt]{\tiny + 50 names not said}};
\begin{scope}[shift={(6.8,-6.25)}]
  \foreach \r in {0,...,3} {\foreach \c in {0,...,24} {\node[cell, fill=black!8] at ({\c*0.26},{-\r*0.22}) {};}}
  \foreach \c/\r in {2/1,3/0,5/2,7/3,9/1,10/1,12/0,14/2,15/2,17/3,19/1,21/0,22/2,24/1} {\node[cell, fill=black!22] at ({\c*0.26},{-\r*0.22}) {};}
  % where the name fits: its three pieces at frames 11-14
  \foreach \c/\r in {12/2,13/2,14/3,15/3} {\node[cell, fill=tyAccent!55] at ({\c*0.26},{-\r*0.22}) {};}
  \node[note, anchor=north east] at ({24*0.26+0.13},-0.78) {CTC posteriors};
  % the same name tried at successive positions: two rejected trials (dashed, grey) and the winning one (solid, purple)
  \node[note, anchor=south west, text=black!60] at ({0*0.26-0.14},1.3) {the name tried at successive positions; score = sum of per-frame margins:};
  \foreach \x/\sc/\col/\tc/\st/\verdict in {0/-9.1/black!35/black!45/dashed/poor, 6/-7.4/black!35/black!45/dashed/poor, 12/-0.8/tyAccentDark/tyAccentDark/solid/fits} {
    \draw[\col, thick, \st, rounded corners=2pt] ({\x*0.26-0.14},0.95) rectangle ({\x*0.26+3*0.26+0.14},0.5);
    \node[th, text=\tc] at ({\x*0.26+1.5*0.26},0.72) {เก|ริก|ไกร};
    \node[note, text=\tc, anchor=south] at ({\x*0.26+1.5*0.26},0.98) {\sc\ \verdict};
    \draw[\col, thin, dashed] ({\x*0.26},0.5) -- ({\x*0.26},0.1);
    \draw[\col, thin, dashed] ({\x*0.26+3*0.26},0.5) -- ({\x*0.26+3*0.26},0.1);
  }
  \draw[-{Stealth[length=1.6mm]}, black!55, thick] (-0.6,0.72) -- ({0*0.26-0.3},0.72);
  \draw[-{Stealth[length=1.6mm]}, black!55, thick] ({0*0.26+3*0.26+0.3},0.72) -- ({6*0.26-0.3},0.72);
  \draw[-{Stealth[length=1.6mm]}, black!55, thick] ({6*0.26+3*0.26+0.3},0.72) -- ({12*0.26-0.3},0.72);
  \node[note, anchor=west, text width=2.0cm, align=left] at ({15*0.26+0.35},0.72) {the best position wins};
  \draw[decorate, decoration={brace, amplitude=0.8mm, mirror}, tyAccentDark] ({12*0.26-0.14},-0.85) -- ({15*0.26+0.14},-0.85);
  \node[note, anchor=north, text=tyAccentDark] at ({13.5*0.26},-1.42) {best fit: frame span, score, worst margin};
  % the base text aligned under the frames: the found span sits where the transcript reads the wrong word
  \node[note, anchor=east] at ({12*0.26-1.75},-1.12) {base text:};
  \node[th, anchor=east, text=black!70] at ({12*0.26-0.2},-1.12) {\ldots ที่คุณ};
  \node[th, text=tyWarmDark] at ({13.5*0.26},-1.12) {เกลือไกล};
  \node[th, anchor=west, text=black!70] at ({15*0.26+0.2},-1.12) {เขาบอกว่าน้อง \ldots};
  \draw[tyWarmDark, thin, dashed] ({12*0.26-0.14},-0.95) -- ({12*0.26-0.14},-1.02);
  \draw[tyWarmDark, thin, dashed] ({15*0.26+0.14},-0.95) -- ({15*0.26+0.14},-1.02);
\end{scope}
\node[note, anchor=west, text width=1.5cm, align=left] at (13.75,-6.5) {finds names the transcript lacks};
\end{scope}
\end{scope}
% ======================= row 4: verify
\begin{scope}[yshift=-3.75cm]
\node[srow, minimum height=2.5cm] (r4) at (0,-7.05) {};
\node[what] at (r4.north west) {\stitle{2\quad Verify}\\splice the candidate into the base text; keep it only if the sentence becomes more likely under both heads};
\begin{scope}[yshift=-0.15cm, xshift=0.15cm]
\node[th, anchor=west] at (3.95,-7.45) {คุณ\textcolor{tyWarmDark}{เกลือไกล}เขาบอกว่า};
\node[note, anchor=west] at (3.95,-7.75) {base text};
\node[bar] at (6.3,-7.75) {\phantom{\rule{0.5cm}{1.5mm}}};
\node[th, anchor=west] at (3.95,-8.25) {คุณ\textcolor{tyAccentDark}{\textbf{เกริกไกร}}เขาบอกว่า};
\node[note, anchor=west] at (3.95,-8.55) {with the name};
\node[bar, fill=tyAccent] at (6.3,-8.55) {\phantom{\rule{1.1cm}{1.5mm}}};
\node[font=\scriptsize, text=tyAccentDark] at (7.65,-8.55) {\checkmark};
\node[note, anchor=west] at (8.3,-7.5) {bars: $\log P(\text{text}\mid\text{audio})$ under the transducer and the CTC head};
\node[note, anchor=north west, text width=7.0cm, align=left] at (8.3,-7.7) {an unspoken decoy lowers the likelihood and is dropped; a name already in the transcript in the other script is caught by cross-script similarity\\35 features $\to$ gradient-boosted trees $\to p$; keep if $p \ge \theta$};
\end{scope}
\end{scope}
% ======================= row 5: replace
\begin{scope}[yshift=-4.60cm]
\node[srow, minimum height=1.85cm] (r5) at (0,-9.45) {};
\node[what] at (r5.north west) {\stitle{3\quad Replace}\\map the frame span to characters and write the listed spelling};
\begin{scope}[yshift=-0.15cm, xshift=0.15cm]
\node[th, anchor=west] at (3.95,-9.9) {ตกใจมากเลยที่คุณ\colorbox{tyWarmFill}{\textcolor{tyWarmDark}{เกลือไกล}}เขาบอกว่าน้อง\colorbox{tyWarmFill}{\textcolor{tyWarmDark}{กล้อง}}เป็นลูกของเขาอ่ะ};
\node[th, anchor=west] at (3.95,-10.5) {ตกใจมากเลยที่คุณ\colorbox{tyAccentFill}{\textcolor{tyAccentDark}{\textbf{เกริกไกร}}}เขาบอกว่าน้อง\colorbox{tyAccentFill}{\textcolor{tyAccentDark}{\textbf{ก้อง}}}เป็นลูกของเขาอ่ะ};
\draw[a] (5.0,-10.07) -- (5.0,-10.33);
\node[note, anchor=west, text width=4.3cm, align=left] at (11.2,-10.2) {frame span $\to$ character span via the CTC greedy string, whose characters carry frames; edges snapped};
\end{scope}
\end{scope}
% ======================= spine
\draw[spine] (r1.south -| 1.6,0) -- (r2.north -| 1.6,0);
\draw[spine] (r2.south -| 1.6,0) -- (r3.north -| 1.6,0);
\draw[spine] (r3.south -| 1.6,0) -- (r4.north -| 1.6,0);
\draw[spine] (r4.south -| 1.6,0) -- (r5.north -| 1.6,0);
\end{tikzpicture}
\caption{\textbf{\sysname on the two heads of \hyb}, step by step on the
second utterance of \Cref{fig:hero}. One encoder pass feeds both heads.
The transducer head gives the base text, which is the output when no list
is given. With a list, each listed name is laid over the CTC posteriors
and its best path through the frames is found (1); the candidate is
spliced into the base text and kept if the sentence becomes more likely
under both heads (2); and the located span of the base text is replaced
by the listed spelling (3). Stages 1 to 3 run on CPU.}
\label{fig:system}
\end{figure}

